Concurrency Models with Causality and Events as Psi-calculi

Psi-calculi are a parametric framework for nominal calculi, where standard calculi are found as instances, like the pi-calculus, or the cryptographic spi-calculus and applied-pi. Psi-calculi have an interleaving operational semantics, with a strong foundation on the theory of nominal sets and process algebras. Much of the expressive power of psi-calculi comes from their logical part, i.e., assertions, conditions, and entailment, which are left quite open thus accommodating a wide range of logics. We are interested in how this expressiveness can deal with event-based models of concurrency. We thus take the popular prime event structures model and give an encoding into an instance of psi-calculi. We also take the recent and expressive model of Dynamic Condition Response Graphs (in which event structures are strictly included) and give an encoding into another corresponding instance of psi-calculi. The encodings that we achieve look rather natural and intuitive. Additional results about these encodings give us more confidence in their correctness.

==> eptcsdata.tex <==
\providecommand{\firstpage}{4}
\providecommand{\publicationstatus}{I. Lanese, A. Lluch Lafuente, A. Sokolova, H. T. Vieira (Eds.):\\
7th Interaction and Concurrency Experience (ICE 2014)\\
EPTCS 166, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.166.3}{10.4204/EPTCS.166.3}}

